DR-Tools: a suite of lightweight open-source tools to measure and visualize Java source code

In Software Engineering, some of the most critical activities are maintenance and evolution. However, to perform both with quality, minimizing impacts and risks, developers need to analyze and identify where the main problems come from previously. In this paper, we introduce DR-Tools Suite, a set of lightweight open-source tools that analyze and calculate source code metrics, allowing developers to visualize the results in different formats and graphs. Also, we define a set of heuristics to help the code analysis. We conducted two case studies (one academic and one industrial) to collect feedback on the tools suite, on how we will evolve the tools, as well as insights to develop new tools that support developers in their daily work.

==> 30Background.tex <==
\section{Background}
\label{sec:background}

Metrics measure specific properties of a software system, mapped by numbers or indicators, according to well-defined rules for measurement objectives. 
The measurement is used to describe, judge, or even predict software system characteristics \cite{Lanza:2003}.
According to Mathias \al \cite{Mathias:1999}, the metrics generated by combining different information extracted from the software, to guide and qualify the analyzed software itself. 
Several studies exploring metrics in different contexts like complexity \cite{McCabe:1976}, object-oriented \cite{Lanza:2010}, cohesion/coupling \cite{Bob:2007}, architecture \cite{Koziolek:2011}, among others. 
The metrics also used as an approach to smell detection \cite{Bigonha:2019}, fault prediction \cite{Radjenovic:2013}, and managing the technical debt \cite{Charalampidou:2019}.

With the popularity of metrics, numerous tools have emerged, commercial\footnote{\url{https://scitools.com/}} or open-source\footnote{\url{https://github.com/mauricioaniche/ck}}, with different features and purposes. 
Studies such as \cite{Bakar:2012} conducted studies are comparing various metric tools, noting that even using the same metrics, they obtained different results.

Some of these reasons are the inconsistency of nomenclatures (same names and different meanings for the same metric), and similar meanings (with different names for the same metric), discussed in more detail in \cite{Saraiva:2014}.
Some important things to consider when developing tools are correlating metrics with quality attributes \cite{Lincke:2008}, using thresholds to predict bugs and smells \cite{Bigonha:2019}, and which metrics are effectively applied to a real scenario \cite{Bouwers:2013}.
